Unsupervised Numerical Reasoning to Extract Phenotypes from Clinical Text by Leveraging External Knowledge

Extracting phenotypes from clinical text has been shown to be useful for a variety of clinical use cases such as identifying patients with rare diseases. However, reasoning with numerical values remains challenging for phenotyping in clinical text, for example, temperature 102F representing Fever. Current state-of-the-art phenotyping models are able to detect general phenotypes, but perform poorly when they detect phenotypes requiring numerical reasoning. We present a novel unsupervised methodology leveraging external knowledge and contextualized word embeddings from ClinicalBERT for numerical reasoning in a variety of phenotypic contexts. Comparing against unsupervised benchmarks, it shows a substantial performance improvement with absolute gains on generalized Recall and F1 scores up to 79% and 71%, respectively. In the supervised setting, it also surpasses the performance of alternative approaches with absolute gains on generalized Recall and F1 scores up to 70% and 44%, respectively.

==> sections/others.tex <==
% \section{Ethics Considerations}
% The research has been carried out in accordance with relevant guidelines and regulations for the MIMIC-III data. Clinical experts received consulting fees for annotating data and validating the external knowledge for numerical reasoning. The main objective of the proposed model is to extract phenotypic information from unstructured clinical notes to assist clinicians in their decisions. Before the deployment of the propose method in the actual clinical setting, the proposed method is subject to systematic debugging, extensive simulation, testing and validation under the supervision of expert clinicians following related regulatory guidelines.

% \section{Code and Data Availability}
% The MIMIC-III dataset is publicly available at \url{https://mimic.mit.edu/} (accessed in November 2021). The code, gold labels and other data could not be shared publicly due to its proprietary nature. The implementation details are described in Section \ref{subsec:implementation_details}.

% \section{Competing Interests}
% Vibhor Gupta, Yike Guo and Jingqing Zhang are founders and co-founders of Pangaea Data Limited. Julia Ive is a consulting advisor to Pangaea Data Limited. Ashwani Tanwar is employed by Pangaea Data Limited. This work is under collaboration with Pangaea Data Limited, Imperial College London, Queen Mary University of London, Hong Kong Baptist University.

% \section{Funding}
% This research is solely funded by Pangaea Data Limited.

% \section{Author Contributions}
% \textbf{Ashwani Tanwar}: Conceptualization, Methodology, Software, Validation, Investigation, Writing Manuscript.
% \textbf{Jingqing Zhang}: Conceptualization, Methodology, Resources, Data Curation, Writing Manuscript.
% \textbf{Julia Ive}: Conceptualization, Methodology, Writing Manuscript, Review.
% \textbf{Vibhor Gupta}: Conceptualization, Review, Supervision, Project Administration.
% \textbf{Yike Guo}: Conceptualization, Review, Supervision, Project Administration.

\section{Acknowledgements}
We would like to thank Dr. Garima Gupta, Dr. Deepa (M.R.S.H) and Dr. Ashok (M.S.) for helping us create gold-standard phenotype annotation data and validate the external knowledge for numerical reasoning. 
